Optimal Power Flow as a Polynomial Optimization Problem

Formulating the alternating current optimal power flow (ACOPF) as a polynomial optimization problem makes it possible to solve large instances in practice and to guarantee asymptotic convergence in theory.

==> LL_Duality_Proof.tex <==
% \begin{IEEEproof}[Proof of Proposition \ref{thm:LavaeiLowBad}]
% %\begin{proof}
% Let us consider a system, where there is one slack bus and the total demand for real power across all buses is $d$.
% The one slack bus 
% corresponds to a generator with the upper bound of $\overline P_1$ on the active power produced and a link to another power system, where the price is given by the supply and demand in an open market.
% %\textcolor{red}{$=$ sum of apparent power over all buses?}
% The equalities of [PP4] can be cast as a natural multihomogenous structure of multidegree $(1,1)$.  Since the slack bus voltage is fixed at a reference value, the system has $2n-2$ such equations in $(n-1, n-1)$ variables. By the multihomogeneous form of Bezout's Theorem (see e.g. Theorem 8.4.7 in \cite{Sommese2005}), the total number of complex solutions to the equalities of
% [PP4] is finite. 
% %Further, notice that, if there are any feasible solutions, there are an even number of them.
% % by Lemma~\ref{thm:evenRoots}.
% If there are at least two real solution $x^+$, $x^*$, 
% such as in the well-known two-bus instance of \cite{Bukhsh2013},
% such that loss($x^+$) $-$ loss($x^*$) $= \epsilon$, 
% one may consider the cost function for the open market to be 
% piece-wise exponential function in the demand for real power $P_2$.
% For instance, from some threshold $d - \overline P_1 - \epsilon$, one use $P_2^\epsilon$ to obtain the result.
% 
% %\end{proof}
% Although the instance used in the proof is somewhat contrived, notice that economic theory does suggest that prices may be exponential in demands. 
% 
% \end{IEEEproof}
%\begin{IEEEproof}[Proof of Proposition \ref{thm:LavaeiLowBad}]
\begin{proof}
Let us consider a system, where there is one slack bus and the Lavaei-Low relaxation [OPF-SDP]  \cite{lavaei2012zero} does produce objective function value $z \ge 1$, which is not the global optimum $f(x^*)$.
For example, this could be the two-bus instance of \cite{Bukhsh2013}.
We can produce a variant of the instance with a new objective function given by
$f'(\cdot ) := C(k) f(\cdot)$, i.e. changing the $c^0_i, c^1_i, c^2_i$ for each generator $i$, to obtain the result when choosing $C(k)$ sufficiently large.
\end{proof}
%\end{IEEEproof}

==> PP_Dense_proof.tex <==
%\section{Proofs}
\appendix
\begin{proof}[Proof of Theorem \ref{thm:equivalence}]
%\section{Proofs}
%$\begin{proof}[Proof of Theorem \ref{thm:equivalence}]
Notice that the variables in [OP$_2$] are $x$, $P^g_k$, and $P_{lm}$ and $Q_{lm}$. However, not all the monomials appear in the polynomial formulation and hence using the first level of the hierarchy, $\mathcal{{K}}^{r}_G$, where $r=2$ one can approximate [OP$_2$]:{\small
\begin{align*}
\begin{split}
\max \quad & \varphi \\
\stt & \sum_{k\in G} \left(c^2_k(P_k^g)^2+c^1_k(P_k^d + \text{tr}(Y_kxx^T))+c^0_k\right) - \varphi \\
&= A(x) + \sum_{k\in G}B_k(P^g_k)+ \sum_{(l,m) \in L}C_{lm}(P_{lm},Q_{lm}) \\
&+ \sum_{k \in N} \overline{\lambda}_k( P_k^{\max}-P_k^d -\text{tr}(Y_kxx^T)) \\ &
+ \sum_{k \in N} \underline{\lambda}_k( -P_k^{\min}+P_k^d +\text{tr}(Y_kxx^T)) \\
&+ \sum_{k \in N} \overline{\gamma}_k( Q_k^{\max}-Q_k^d -\text{tr}(\bar{Y}_kxx^T)) \\
&+ \sum_{k \in N} \underline{\gamma}_k( -Q_k^{\min}+Q_k^d +\text{tr}(\bar{Y}_kxx^T)) \\
& +\sum_{k \in N} \overline{\mu}_k( (V_k^{\max})^2-\text{tr}(M_kxx^T))  \\
&+ \sum_{k \in N} \underline{\mu}_k( (-V_k^{\min})^2+\text{tr}(M_kxx^T)) \\
& +\sum_{(l,m) \in L} a_{lm} ((S_{lm}^{\max})^2  -P_{lm}^2-Q_{lm}^2) \\
&+  \sum_{k \in G}b_k (P^g_k-  \text{tr}(Y_kxx^T)-P_k^d) \\
& +\sum_{(l,m) \in L} c_{lm} (P_{lm} - \text{tr}(Y_{lm}xx^T))\\
&+\sum_{(l,m) \in L} d_{lm} (Q_{lm} - \text{tr}(\bar{Y}_{lm}xx^T))
\end{split}
\end{align*}}
where $A(x), B_k(P^g_k), C_{lm}(P_{lm},Q_{lm})$ are polynomials that are sum of squares as a function of $x$, $P^g_k$, and $P_{lm}$ and $Q_{lm}$ respectively. That is $A(x)=xAx^T$, $B_k(P^g_k)=  \left[ \begin{matrix} 1 \\ P^g_k \end{matrix}  \right]B_k  \left[ \begin{matrix} 1 \\ P^g_k \end{matrix}  \right]^T,$ and $C_{lm}(P_{lm},Q_{lm})=  \left[ \begin{matrix} 1 \\ P_{lm} \\ Q_{lm} \end{matrix}  \right] C_{lm} \left[ \begin{matrix} 1 \\ P_{lm} \\ Q_{lm} \end{matrix}  \right]^T,$ where $A, B_k,$ and $C_{lm}$ are positive semidefinite matrices of dimension $2|N|\times 2|N|$, $2\times 2$ and $3\times 3$ respectively. The variables $\overline{\lambda}_k, \underline{\lambda}_k, \overline{\gamma}_k, \underline{\gamma}_k, \overline{\mu}_k, \underline{\mu}_k$, and $a_{lm}$,are non-negative variables and $b_k, c_{lm},$ and $d_{lm}$ are free variables. By equating the coefficients of the monomials of the above problem, %we rewrite it as{\small
% \begin{align*}
% \begin{split}
% \max  \quad& \varphi \\
% \stt & \sum_{k \in G} c^1_kP^d_k +\sum_{k \in G} c^0_k - \varphi \\
% &= \sum_{k\in G}B_k^{00}+ \sum_{(l,m) \in L}C_{lm}^{00} + \sum_{k \in N} \overline{\lambda}_k (P_k^{\max}-P_k^d )  \\
% &  + \sum_{k \in N} \underline{\lambda}_k( -P_k^{\min}+P_k^d )+ \sum_{k \in N} \overline{\gamma}_k( Q_k^{\max}-Q_k^d ) \\
% &+ \sum_{k \in N} \underline{\gamma}_k( -Q_k^{\min}+Q_k^d )   + \sum_{k \in N} \overline{\mu}_k( V_k^{\max})^2 \\
% &- \sum_{k \in N} \underline{\mu}_k(V_k^{\min})^2 + \sum_{(l,m) \in L} a_{lm}(S_{lm}^{\max})^2- \sum_{k\in G}b_kP_k^d \\
%  & \sum_{k \in N}c_1^k Y_k = A-\sum_{k \in N}\left(\overline{\lambda}_k Y_k +\underline{\lambda}_k Y_k -\overline{\gamma}_k \bar{Y}_k \right. \\& +\left.\underline{\gamma}_k \bar{Y}_k - \overline{\mu}_k (V_k^{\max})^2   +\underline{\mu}_k (V_k^{\min})^2 - b_k Y_k \right) \\&-\sum_{(l,m) \in L} \left( c_{lm} Y_{lm}  + d_{lm} \bar{Y}_{lm} \right)\\
%  & 0 = 2B^{12}_k+b_k \qquad c_k^2 = B^{22}_k \\
%  & 0 = c_{lm} +2C_{lm}^{12} \qquad 0 = d_{lm} +2C_{lm}^{13} \\
%   & 0 = 2C_{lm}^{23} \qquad\qquad\quad  0=-a_{lm}+ C^{22}_{lm} \\& 0 = -a_{lm} +C^{33}_{lm}  \\
%   & A, B_k, C_{lm} \succeq 0.
%   \end{split}
% \end{align*}}
and substituting some of the variables:{\small
\begin{align*}
\begin{split}
\textbf{[PP2-H1] }\\
\max  \quad& \sum_{k \in G} c^1_kP^d_k +\sum_{k \in G} c^0_k -\sum_{k\in G}B_k^{00}- \sum_{(l,m) \in L}C_{lm}^{00} \\
&- \sum_{k \in N} \overline{\lambda}_k (P_k^{\max}-P_k^d )    - \sum_{k \in N} \underline{\lambda}_k( -P_k^{\min}+P_k^d )\\
&- \sum_{k \in N} \overline{\gamma}_k( Q_k^{\max}-Q_k^d ) - \sum_{k \in N} \underline{\gamma}_k( -Q_k^{\min}+Q_k^d ) \\
&  - \sum_{k \in N} \overline{\mu}_k( V_k^{\max})^2 +\sum_{k \in N} \underline{\mu}_k(V_k^{\min})^2 \\
&- \sum_{(l,m) \in L}  C^{22}_{lm}(S_{lm}^{\max})^2 -\sum_{k\in G} 2B^{12}_kP_k^d \\
\stt & A = \sum_{k \in N} \left(c_1^k Y_k +\overline{\lambda}_k Y_k -\underline{\lambda}_k Y_k +\overline{\gamma}_k \bar{Y}_k \right. \\
&\left. -\underline{\gamma}_k \bar{Y}_k+ \overline{\mu}_k (V_k^{\max})^2 -\underline{\mu}_k (V_k^{\min})^2 -2B^{12}_k Y_k \right) \\
&- \sum_{(l,m) \in L} \left(2C_{lm}^{12} Y_{lm}  +2C_{lm}^{13} \bar{Y}_{lm}\right) \\
  &c_k^2 = B^{22}_k \qquad 0 = 2C_{lm}^{23} \\
  & C^{22}_{lm}- C^{33}_{lm} =0 \\
  & A, B_k, C_{lm} \succeq 0.
  \end{split}
\end{align*}}
which is equivalent to optimization problem 4 described in \cite{lavaei2012zero} (i.e., the dual of [OP-SDP]) and exhibits the same structure.\end{proof} %Hence we apply two techniques to improve on the bounds obtained by [D]. The first approach is discussed int he next section where valid inequalities are added to [PP2] which are translated to more variables to [D]. The resulting scheme improves the [D] relaxation and hence the bound. In the second approach, we exploit the sparsity pattern of the two polynomial programs [PP2] and [PP4] to provide global optimal solutions for the OPF problem.
%\end{proof}

% Notice that the variables in [OPF-PP2] are $x$, $P_k$, and $P_{lm}$ and $Q_{lm}$. However, not all the monomials appear in the polynomial formulation and hence using the first level of the hierarchy, $\mathcal{{K}}^{r}_G$, where $r=2$ one can approximate [OPF-PP2]:
% \begin{align*}
% \max & \varphi \\
%  & \sum_{k\in G} \left(c^2_kP_k^2+c^1_k(P_k^d + \text{tr}(Y_kxx^T))+c^0_k\right) - \varphi = A(x) + \sum_{k\in G}B_k(P_k)+ \sum_{(l,m) \in L}C_{lm}(P_{lm},Q_{lm}) \\
% &+ \sum_{k \in N} \overline{\lambda}_k( P_k^{\max}-P_k^d -\text{tr}(Y_kxx^T)) + \sum_{k \in N} \underline{\lambda}_k( -P_k^{\min}+P_k^d +\text{tr}(Y_kxx^T)) \\
% &+ \sum_{k \in N} \overline{\gamma}_k( Q_k^{\max}-Q_k^d -\text{tr}(\bar{Y}_kxx^T)) + \sum_{k \in N} \underline{\gamma}_k( -Q_k^{\min}+Q_k^d +\text{tr}(\bar{Y}_kxx^T)) \\
% & +\sum_{k \in N} \overline{\mu}_k( (V_k^{\max})^2-\text{tr}(M_kxx^T)) + \sum_{k \in N} \underline{\mu}_k( (-V_k^{\min})^2+\text{tr}(M_kxx^T)) \\
% & +\sum_{(l,m) \in L} a_{lm} ((S_{lm}^{\max})^2  -P_{lm}^2-Q_{lm}^2) +  \sum_{k \in G}b_k (P_k-  \text{tr}(Y_kxx^T)-P_k^d) \\
% & +\sum_{(l,m) \in L} c_{lm} (P_{lm} - \text{tr}(Y_{lm}xx^T)) +\sum_{(l,m) \in L} d_{lm} (Q_{lm} - \text{tr}(\bar{Y}_{lm}xx^T))
% \end{align*}
% where $A(x), B_k(P_k), C_{lm}(P_{lm},Q_{lm})$ are polynomials that are sum of squares as a function of $x$, $P_k$, and $P_{lm}$ and $Q_{lm}$ respectively. That is $A(x)=xAx^T$, $B_k(P_k)=  \left[ \begin{matrix} 1 \\ P_k \end{matrix}  \right]B  \left[ \begin{matrix} 1 \\ P_k \end{matrix}  \right]^T,$ and $C_{lm}(P_{lm},Q_{lm})=  \left[ \begin{matrix} 1 \\ P_{lm} \\ Q_{lm} \end{matrix}  \right]B  \left[ \begin{matrix} 1 \\ P_{lm} \\ Q_{lm} \end{matrix}  \right]^T,$ where $A, B_k,$ and $C_{lm}$ are positive semidefinite matrices of dimension $2|N|\times 2|N$, $2\times 2$ and $3\times 3$ respectively. The variables $\overline{\lambda}_k, \underline{\lambda}_k, \overline{\gamma}_k, \underline{\gamma}_k, \overline{\mu}_k, \underline{\mu}_k$ and $a_{lm}$ are non-negative variables. By equating the coefficients of the monomials of the above problem, we rewrite it as
% \begin{align*}
% \max  \quad& \varphi \\
%  & \sum_{k \in G} c^1_kP^d_k +\sum_{k \in G} c^0_k - \varphi = \sum_{k\in G}B_k^{00}+ \sum_{(l,m) \in L}C_{lm}^{00} + \sum_{k \in N} \overline{\lambda}_k (P_k^{\max}-P_k^d )  \\
% &  + \sum_{k \in N} \underline{\lambda}_k( -P_k^{\min}+P_k^d )+ \sum_{k \in N} \overline{\gamma}_k( Q_k^{\max}-Q_k^d ) + \sum_{k \in N} \underline{\gamma}_k( -Q_k^{\min}+Q_k^d ) \\
% &  + \sum_{k \in N} \overline{\mu}_k( V_k^{\max})^2 - \sum_{k \in N} \underline{\mu}_k(V_k^{\min})^2 + \sum_{(l,m) \in L} a_{lm}(S_{lm}^{\max})^2+ \sum_{k\in G}b_kP_k^d \\
%  & c_1^k Y_k = A_k -\overline{\lambda}_k Y_k +\underline{\lambda}_k Y_k -\overline{\gamma}_k \bar{Y}_k +\underline{\gamma}_k \bar{Y}_k - \overline{\mu}_k (V_k^{\max})^2 \\& +\underline{\mu}_k (V_k^{\min})^2 - b_k Y_k - c_{lm} Y_{lm}  - d_{lm} \bar{Y}_{lm} \\
%  & 0 = 2B^{12}_k+b_k \\
%   &c_k^2 = B^{22}_k \\
%  & 0 = c_{lm} +2C_{lm}^{12}\\
%   & 0 = d_{lm} +2C_{lm}^{13} \\
%   & 0 = 2C_{lm}^{23} \\
%   & 0=-a_{lm}+ C^{22}_{lm} \\
%   & 0 = -a_{lm} +C^{33}_{lm} 
% \end{align*}
% \begin{align*}
% \textbf{[D] } & \notag \\
% \max  \quad& \sum_{k \in G} c^1_kP^d_k +\sum_{k \in G} c^0_k -\sum_{k\in G}B_k^{00}- \sum_{(l,m) \in L}C_{lm}^{00} - \sum_{k \in N} \overline{\lambda}_k (P_k^{\max}-P_k^d )  \\
% &  - \sum_{k \in N} \underline{\lambda}_k( -P_k^{\min}+P_k^d )- \sum_{k \in N} \overline{\gamma}_k( Q_k^{\max}-Q_k^d ) - \sum_{k \in N} \underline{\gamma}_k( -Q_k^{\min}+Q_k^d ) \\
% &  - \sum_{k \in N} \overline{\mu}_k( V_k^{\max})^2 +\sum_{k \in N} \underline{\mu}_k(V_k^{\min})^2 - \sum_{(l,m) \in L}  C^{22}_{lm}(S_{lm}^{\max})^2 +\sum_{k\in G} 2B^{12}_kP_k^d \\
%  & A_k = c_1^k Y_k +\overline{\lambda}_k Y_k -\underline{\lambda}_k Y_k +\overline{\gamma}_k \bar{Y}_k -\underline{\gamma}_k \bar{Y}_k+ \overline{\mu}_k (V_k^{\max})^2 \\& -\underline{\mu}_k (V_k^{\min})^2 -2B^{12}_k Y_k -2C_{lm}^{12} Y_{lm}  -2C_{lm}^{13} \bar{Y}_{lm} \\
%   &c_k^2 = B^{22}_k \\
%    & 0 = 2C_{lm}^{23} \\
%   & C^{22}_{lm}- C^{33}_{lm} =0
% \end{align*}
% which is very similar to optimization problem 4 described in \cite{lavaei2012zero} (i.e., the dual of [OPF-SDP]) and exhibits the same structure. Hence we apply two techniques to improve on the bounds obtained by [OPF-D]. The first approach is discussed int he next section where valid inequalities are added to [OPF-PP2] which are translated to more variables to [OPF-D]. The resulting scheme improves the [OPF-D] relaxation and hence the bound. In the second approach, we exploit the sparsity pattern of the two polynomial programs [OPF-PP2] and [OPF-PP4] to provide global optimal solutions for the OPF problem.


